Beauville-Laszlo gluing of algebraic spaces

For a complete discrete valuation field $K$, we show that one may always glue a separated formal algebraic space $\mathfrak{X}$ over $\mathcal{O}_K$ to a separated algebraic space $U$ over $K$ along an open immersion of rigid spaces $j\colon \mathfrak{X}^{\rm rig}\to U^{\rm an}$, producing a separated algebraic space $X$ over $\mathcal{O}_K$. This process gives rise to an equivalence between such `gluing triples' $(U,\mathfrak{X},j)$ and separated algebraic spaces $X$ over $\mathcal{O}_K$, which one might interpret as a version of the Beauville--Laszlo theorem for algebraic spaces rather than coherent sheaves. Moreover, an analogous equivalence exists over any excellent base. Examples due to Matsumoto imply that the result of such a gluing might be a genuine algebraic space (not a scheme) even if $U$ and the special fiber of $\mathfrak{X}$ are projective. The proof is a combination of Nagata compactification theorem for algebraic spaces and of Artin's contraction theorem. We give multiple examples and applications of this idea.

==> friedegg.tex <==
\usetikzlibrary {arrows.meta,bending,positioning}
\usetikzlibrary{decorations.pathreplacing}
\begin{tikzpicture} 
    % \newlength{\mywidth}
    % \setlength{\mywidth}{3cm}
    % \clip (-\mywidth,-\mywidth-1cm) rectangle + (2*\mywidth,2*\mywidth+1cm);
    
    \node[inner sep=0pt] at (0,0) {\includegraphics[width=.35\textwidth]{figure.jpg}};
    
    \node at (-.9,2.1) {$U$}; % before at (-1.7,2.1) % or $X^\circ;
    \node at (1.6,1.4) {$\mathfrak{X}_0$}; % before at (2,1.1) % or X_0
    \node at (-.9, -3.2) {$S^\circ$}; % or S^\circ={\rm Spec}(K)
    \node at (1.6, -3.2) {$S_0$}; % or S_0={\rm Spec}(k)
    \node (A) at (-2, -.7) {$\mathfrak{X}^{\rm rig}$}; % or \widehat{X}^{\rm rig}
    \node (B) at (-.8,.3) {};
    \draw [thick] (A) edge [->,bend left=45] (B);
    \draw [decorate,decoration={brace,amplitude=5pt,mirror,raise=4ex},thick] (-.9,.1) -- (1.4,.1) node[midway,yshift=-3em]{$\mathfrak{X}$}; % or \widehat{X}
    \fill[white] (.1-0.3,.5+0.3) rectangle + (0.6, -0.5);
    \node at (.1, .5) {${\rm sp}_{\mathfrak{X}}$}; % positioned at (.6,1.55) before % {\rm sp}_{\widehat{X}} (or without subscript)
\end{tikzpicture}

